Enhancing Network Management Using Code Generated by Large Language Models

Analyzing network topologies and communication graphs plays a crucial role in contemporary network management. However, the absence of a cohesive approach leads to a challenging learning curve, heightened errors, and inefficiencies. In this paper, we introduce a novel approach to facilitate a natural-language-based network management experience, utilizing large language models (LLMs) to generate task-specific code from natural language queries. This method tackles the challenges of explainability, scalability, and privacy by allowing network operators to inspect the generated code, eliminating the need to share network data with LLMs, and concentrating on application-specific requests combined with general program synthesis techniques. We design and evaluate a prototype system using benchmark applications, showcasing high accuracy, cost-effectiveness, and the potential for further enhancements using complementary program synthesis techniques.

==> tables/malt_sum_table.tex <==
\begin{table}
\fontsize{9pt}{9pt}\selectfont
\centering
\tightcaption{Summary for MALT}
\resizebox{0.6\columnwidth}{!}{
\begin{tblr}{
  row{1} = {c},
  cell{2}{2} = {c},
  cell{2}{3} = {c},
  cell{2}{4} = {c},
  cell{3}{2} = {c},
  cell{3}{3} = {c},
  cell{3}{4} = {c},
  cell{4}{2} = {c},
  cell{4}{3} = {c},
  cell{4}{4} = {c},
  cell{5}{2} = {c},
  cell{5}{3} = {c},
  cell{5}{4} = {c},
  hline{1-2,6} = {-}{},
}
                 & SQL  & Pandas & Networkx \\
GPT-4            & 0.11 & 0.56   & \textbf{0.78}     \\
GPT-3            & 0.11 & \textbf{0.44}   & \textbf{0.44}     \\
text-davinci-003 & 0.11 & 0.22   & \textbf{0.56}    \\
Google Bard      & 0.0  & 0.11   & \textbf{0.33}     
\end{tblr}
}
\label{tab::sum_malt}
\end{table}

==> tables/seg_sum_table.tex <==
% \usepackage{tabularray}
\begin{table}
\centering
\tightcaption{Summary for Traffic Analysis}
\resizebox{0.65\columnwidth}{!}{
\begin{tblr}{
  row{1} = {c},
  cell{2}{2} = {c},
  cell{2}{3} = {c},
  cell{2}{4} = {c},
  cell{2}{5} = {c},
  cell{3}{2} = {c},
  cell{3}{3} = {c},
  cell{3}{4} = {c},
  cell{3}{5} = {c},
  cell{4}{2} = {c},
  cell{4}{3} = {c},
  cell{4}{4} = {c},
  cell{4}{5} = {c},
  cell{5}{2} = {c},
  cell{5}{3} = {c},
  cell{5}{4} = {c},
  cell{5}{5} = {c},
  hline{1-2,6} = {-}{},
}
                 & Strawman & SQL  & Pandas & Networkx \\
GPT-4            & 0.29     & 0.5  & 0.38   & \textbf{0.88}     \\
GPT-3          & 0.17     & 0.13 & 0.25   & \textbf{0.63}     \\
text-davinci-003 & 0.21     & 0.29 & 0.29   & \textbf{0.63}     \\
Google Bard      & 0.04     & 0.08 & 0.08   & \textbf{0.42}     
\end{tblr}
}
\label{tab::sum_traffic}
\end{table}

==> tables/self_consistency.tex <==
\begin{table}
\centering
\caption{Pass@k Improvement on All of MALT Queries}
\resizebox{0.5\columnwidth}{!}{
\begin{tabular}{cccc} 
\hline
                                                         & SQL & Pandas & Networkx  \\ 
\hline
Google Bard~                                                 & 0.0   & 0.11      & 0.33         \\
\begin{tabular}[c]{@{}c@{}}Google Bard\\with Pass@k\end{tabular} & \textbf{0.22}   & \textbf{0.33}      & \textbf{0.78}         \\
\hline
\end{tabular}
}
\label{tab::self_consistency}
\end{table}

==> tables/self_debug.tex <==
\begin{table}
\centering
\caption{Self-debugging Improvement on Failed Examples}
\resizebox{0.5\columnwidth}{!}{
\begin{tabular}{cccc} 
\hline
                & SQL & Pandas & Networkx  \\ 
\hline
Google Bard          & 0.0   & 0.0      & 0.0         \\
\begin{tabular}[c]{@{}c@{}}Google Bard\\with self-debug\end{tabular} & X   & X      & X         \\
\hline
\end{tabular}
}
\label{tab::self_debug}
\end{table}

==> tables/table_basic_MALT.tex <==
% \usepackage{tabularray}
\begin{table}
\centering
\caption{Breakdown for MALT}
\resizebox{\columnwidth}{!}{
\begin{tblr}{
  row{1} = {c},
  row{2} = {c},
  cell{1}{2} = {c=3}{},
  cell{1}{5} = {c=3}{},
  cell{1}{8} = {c=3}{},
  cell{3}{2} = {c},
  cell{3}{3} = {c},
  cell{3}{4} = {c},
  cell{3}{5} = {c},
  cell{3}{6} = {c},
  cell{3}{7} = {c},
  cell{3}{8} = {c},
  cell{3}{9} = {c},
  cell{3}{10} = {c},
  cell{4}{2} = {c},
  cell{4}{3} = {c},
  cell{4}{4} = {c},
  cell{4}{5} = {c},
  cell{4}{6} = {c},
  cell{4}{7} = {c},
  cell{4}{8} = {c},
  cell{4}{9} = {c},
  cell{4}{10} = {c},
  cell{5}{2} = {c},
  cell{5}{3} = {c},
  cell{5}{4} = {c},
  cell{5}{5} = {c},
  cell{5}{6} = {c},
  cell{5}{7} = {c},
  cell{5}{8} = {c},
  cell{5}{9} = {c},
  cell{5}{10} = {c},
  cell{6}{2} = {c},
  cell{6}{3} = {c},
  cell{6}{4} = {c},
  cell{6}{5} = {c},
  cell{6}{6} = {c},
  cell{6}{7} = {c},
  cell{6}{8} = {c},
  cell{6}{9} = {c},
  cell{6}{10} = {c},
  hline{1,3,7} = {-}{},
}
                 & SQL   &       &       & Pandas &       &       & Networkx &       &       \\
                 & E (3) & M (3) & H (3) & E (3)  & M (3) & H (3) & E (3)    & M (3) & H (3) \\
GPT-4            & 0.33  & 0.0  & 0.0      & 0.67    & 0.67   & 0.33  & 1.0      & 1.0   & 0.33  \\
GPT-3          & 0.33  & 0.0  & 0.0      & 0.67       &  0.67     & 0.0      & 0.67      & 0.67  & 0.0  \\
text-davinci-003 & 0.33  & 0.0   & 0.0   & 0.33   & 0.33  & 0.0   & 0.67      & 0.67  & 0.33  \\
Google Bard      & 0.0   & 0.0  & 0.0   & 0.33   & 0.0   & 0.0   & 0.67     & 0.33  & 0.0  
\end{tblr}
}
\label{tab::breakdown_malt}
\end{table}

==> tables/table_basic_micro-seg.tex <==
% \usepackage{tabularray}
\begin{table}
\fontsize{15pt}{15pt}
\centering
\caption{Breakdown for Traffic Analysis}
\resizebox{\columnwidth}{!}{
\begin{tblr}{
  row{1} = {c},
  row{2} = {c},
  cell{1}{2} = {c=3}{},
  cell{1}{5} = {c=3}{},
  cell{1}{8} = {c=3}{},
  cell{1}{11} = {c=3}{},
  cell{3}{2} = {c},
  cell{3}{3} = {c},
  cell{3}{4} = {c},
  cell{3}{5} = {c},
  cell{3}{6} = {c},
  cell{3}{7} = {c},
  cell{3}{8} = {c},
  cell{3}{9} = {c},
  cell{3}{10} = {c},
  cell{3}{11} = {c},
  cell{3}{12} = {c},
  cell{3}{13} = {c},
  cell{4}{2} = {c},
  cell{4}{3} = {c},
  cell{4}{4} = {c},
  cell{4}{5} = {c},
  cell{4}{6} = {c},
  cell{4}{7} = {c},
  cell{4}{8} = {c},
  cell{4}{9} = {c},
  cell{4}{10} = {c},
  cell{4}{11} = {c},
  cell{4}{12} = {c},
  cell{4}{13} = {c},
  cell{5}{2} = {c},
  cell{5}{3} = {c},
  cell{5}{4} = {c},
  cell{5}{5} = {c},
  cell{5}{6} = {c},
  cell{5}{7} = {c},
  cell{5}{8} = {c},
  cell{5}{9} = {c},
  cell{5}{10} = {c},
  cell{5}{11} = {c},
  cell{5}{12} = {c},
  cell{5}{13} = {c},
  cell{6}{2} = {c},
  cell{6}{3} = {c},
  cell{6}{4} = {c},
  cell{6}{5} = {c},
  cell{6}{6} = {c},
  cell{6}{7} = {c},
  cell{6}{8} = {c},
  cell{6}{9} = {c},
  cell{6}{10} = {c},
  cell{6}{11} = {c},
  cell{6}{12} = {c},
  cell{6}{13} = {c},
  hline{1,3,7} = {-}{},
}
                 & Strawman &        &      & SQL  &        &      & Pandas &        &      & Networkx &        &      \\
                 & E (8) & M (8) & H (8) & E (8)& M (8) & H (8) & E (8)  & M (8)& H (8)& E (8)    & M (8) & H (8)\\
GPT-4            &0.50          & 0.38       & 0.0       & 0.75     &  0.50      & 0.25     & 0.50    & 0.50    & 0.13 & 1.0      & 1.0    & 0.63 \\
GPT-3          &0.38          &0.13       & 0.0     & 0.25     & 0.13       & 0.0     & 0.50       & 0.25       & 0.0     & 1.0      & 0.63   & 0.25 \\
text-davinci-003 & 0.38         &0.25        & 0.0     & 0.63 & 0.25   & 0.0  & 0.63   & 0.25   & 0.0  & 1.0      & 0.75   & 0.13 \\
Google Bard      & 0.25     & 0.0    & 0.0  & 0.25 & 0.0    & 0.0  & 0.25   & 0.0    & 0.0  & 0.88     & 0.25   & 0.13 
\end{tblr}
}
\label{tab::breakdown_traffic}
\end{table}
